REANIMATOR: Reanimate Retrieval Test Collections with Extracted and Synthetic Resources

Retrieval test collections are essential for evaluating information retrieval systems, yet they often lack generalizability across tasks. To overcome this limitation, we introduce REANIMATOR, a versatile framework designed to enable the repurposing of existing test collections by enriching them with extracted and synthetic resources. REANIMATOR enhances test collections from PDF files by parsing full texts and machine-readable tables, as well as related contextual information. It then employs state-of-the-art large language models to produce synthetic relevance labels. Including an optional human-in-the-loop step can help validate the resources that have been extracted and generated. We demonstrate its potential with a revitalized version of the TREC-COVID test collection, showcasing the development of a retrieval-augmented generation system and evaluating the impact of tables on retrieval-augmented generation. REANIMATOR enables the reuse of test collections for new applications, lowering costs and broadening the utility of legacy resources.

==> old_RAG.tex <==

\subsubsection{Query and Data Processing}


\subsubsection{Retrieval and Generation}

We compare the three retrieval setup versions with lexical and semantic retrieval models (BM25 and cosine similarity) based on the CORD-19 qrels.


\subsubsection{Automated Judging}
We follow RAGAS~\cite{es_ragas_2023} and related best practices~\cite{xiong_benchmarking_2024} to assess key aspects such as faithfulness, relevance, and retrieval precision.

\paragraph{RAG Fidelity/Faithfulness Evaluation}
Fidelity and Faithfulness measure how well the generated answer aligns with the retrieved documents and tables~\cite{wang_domainrag_2024, es_ragas_2023}. 
%The approach in \cite{krishna_fact_2024} used up to four documents as context, and increasing the context size showed a performance increase.
Complying with \citet{es_ragas_2023}, we define the answer, denoted as $as(q)$, to be faithful to the context $c(q)$ if the claims made in the answer can be inferred from the context. To estimate faithfulness, we first use an LLM to extract a set of statements, $S(as(q))$. 
The aim of this step is to decompose longer sentences into shorter, more focused assertions. We use the following prompt for this step:
\newline
\textit{Given a question and answer, create one or more statements from each sentence in the given answer. question: [question] answer: [answer]}

\noindent Here, [question] and [answer] refer to the provided question and answer. For each statement $s_i \in S$, the LLM determines if $s_i$ can be inferred from $c(q)$ using a verification function $v(s_i, c(q))$. This verification is carried out using the following prompt:
\newline
\textit{Consider the given context and the following statements, then determine whether they are supported by the information present in the context. Provide a brief explanation for each statement before arriving at the verdict (Yes/No). Provide a final verdict for each statement in order at the end in the given format. Do not deviate from the specified format. statement: [statement 1] ... statement: [statement n]}

\noindent The final faithfulness score, $F$, is computed as 
\[
F = \frac{|V|}{|S|}
\]
where $|V|$ is the number of statements that were supported according to the LLM, and $|S|$ is the total number of statements.

\paragraph{Context Relevance}
The context $c(q)$ is considered relevant to the extent that it exclusively contains the information needed to answer the question \cite{es_ragas_2023}. In particular, this metric aims to penalize the inclusion of redundant information. To estimate context relevance, given a question $q$ and its context $c(q)$, the LLM extracts a subset of sentences, $S_{ext}$, from $c(q)$ that are crucial for answering $q$, using the following prompt:
\newline
\textit{Please extract relevant sentences from the provided context that can potentially help answer the following question. If no relevant sentences are found, or if you believe the question cannot be answered from the given context, return the phrase "Insufficient Information". While extracting candidate sentences, you are not allowed to make any changes to the sentences from the given context.}
\newline
The context relevance score is then computed as 
\[
CR = \frac{\text{number of extracted sentences}}{\text{total number of sentences in } c(q)}
\]

\paragraph{RAG Answer Relevance Evaluation}
This evaluation measures how well the generated answer addresses the input query.

\begin{itemize}
    \item Direct the LLM judge to evaluate how well the generated answer addresses the original query.
    \item Ask for a relevance score, considering both the pertinence and completeness of the response.
\end{itemize}

\noindent \textbf{Approach \cite{es_ragas_2023}}: To estimate answer relevance for a given answer $as(q)$, we prompt the LLM to generate $n$ potential questions $q_i$ based on $as(q)$, as follows:
\newline
\textit{Generate a question for the given answer. answer: [answer]}
\newline
We then obtain embeddings for all generated questions using the \texttt{text-embedding-ada-002} model available from the OpenAI API. For each $q_i$, we calculate the similarity $\mathrm{sim}(q, q_i)$ with the original question $q$, using cosine similarity between the corresponding embeddings. The answer relevance score, $AR$, for question $q$ is computed as
\[
AR = \frac{1}{n} \sum_{i=1}^n \mathrm{sim}(q, q_i)
\]
This metric evaluates how closely the generated answer aligns with the initial question or instruction.

\paragraph{precision, recall}
Further, we report Precision and Recall~\cite{pan_end_end_2022, xiong_benchmarking_2024}.


\subsubsection{Evaluation Process}

Subsequent subsections detail the retrieval process for each condition and outline our evaluation procedures.
We utilize an advanced assessment system incorporating automatic generation and evaluation of nuggets \cite{pradeep_initial_2024}. Based on the taxonomy of \cite{gao_retrieval-augmented_2024}, we apply a naive RAG without pre- and post-retrieval optimization. Many authors present different methods for the individual RAG steps \cite{wang_searching_2024}; however, we focus on strong defaults.


Experiments were conducted in a zero-shot manner~\cite{xiong_benchmarking_2024} but without Multi-Choice Evaluation. We also embed tables as a whole and do not apply advanced table augmentation methods. More sophisticated methods are discussed in \cite{chen_tablerag_2024}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{itemize}
    \item Prompt the LLM judge to compare the generated answer with the retrieved documents and tables.
    \item Ask the judge to score the fidelity on a scale (e.g., 1--5), considering how well the answer reflects the information in the retrieved context.
\end{itemize}

\subsubsection{RAG Accuracy Evaluation or Context Relevance}
This evaluation assesses the correctness of the information provided in the generated answer.


\begin{itemize}
    \item Instruct the LLM judge to assess the factual correctness of the generated answer.
    \item Request a score for accuracy, taking into account any potential hallucinations or misinterpretations of the retrieved information.
\end{itemize}




